Provably Robust DPO: Aligning Language Models with Noisy Feedback

Learning from preference-based feedback has recently gained traction as a promising approach to align language models with human interests. While these aligned generative models have demonstrated impressive capabilities across various tasks, their dependence on high-quality human preference data poses a bottleneck in practical applications. Specifically, noisy (incorrect and ambiguous) preference pairs in the dataset might restrict the language models from capturing human intent accurately. While practitioners have recently proposed heuristics to mitigate the effect of noisy preferences, a complete theoretical understanding of their workings remain elusive. In this work, we aim to bridge this gap by by introducing a general framework for policy optimization in the presence of random preference flips. We focus on the direct preference optimization (DPO) algorithm in particular since it assumes that preferences adhere to the Bradley-Terry-Luce (BTL) model, raising concerns about the impact of noisy data on the learned policy. We design a novel loss function, which de-bias the effect of noise on average, making a policy trained by minimizing that loss robust to the noise. Under log-linear parameterization of the policy class and assuming good feature coverage of the SFT policy, we prove that the sub-optimality gap of the proposed robust DPO (rDPO) policy compared to the optimal policy is of the order $O(\frac{1}{1-2\epsilon}\sqrt{\frac{d}{n}})$, where $\epsilon < 1/2$ is flip rate of labels, $d$ is policy parameter dimension and $n$ is size of dataset. Our experiments on IMDb sentiment generation and Anthropic's helpful-harmless dataset show that rDPO is robust to noise in preference labels compared to vanilla DPO and other heuristics proposed by practitioners.

==> app_new.tex <==
\subsection{Efficient Computation via SGD}

It is evident that computing the exact minimizer $\hat\theta_{\texttt{RR}}$ in~\eqref{eq:robust_rr} is impractical in practice. we replace \eqref{eq:estimator}
by a sequential update rule: 
\begin{align}\label{eq:estimate_SGD}
    \hat \theta_1 = 0~,\,\,\hat\theta_{t+1} = \Pi_{\Theta_B}\Big(\hat\theta_{t} - \eta_t \hat{g}_{t}\Big),\,\, 1\le t \le n~.
\end{align}
Here $\Pi_{\Theta_B}$ is a projection operator onto the set $\Theta_B$, $\eta_t$ is 
a suitable learning rate and $\hat g_{t} = -\nabla_{\hat\theta_t} \log \hat p_{t,\widetilde y_t}$ is the (negative) gradient of the log-predicted score of randomized label $\widetilde y_t$ computed at current estimate $\hat\theta_t$, where $\hat p_{t,y}, y \in {0,1}$ is given by \eqref{eq:predcit_score}.

we can bound the estimation error of $\hat\theta_{\texttt{SGD-RR}}$ in $\ell_2$-norm.

One can also relax this assumption to the population covariance matrix of differential state-action features $x = \phi(s, a^1) - \phi(s, a^0)$, defined as
\begin{align*}
    \Sigma = \mathbb{E}_{s \sim \rho(\cdot), (a^0,a^1)\sim \mu(\cdot | s)} \left[ x x^{\top} \right]~.
\end{align*}
\begin{assumption}[Coverage of feature space]
\label{ass:cov}
The data distributions $\rho,\mu$ are such that $\lambda_{\min}(\Sigma) \ge \kappa$ for some constant $\kappa \!>\! 0$.
\end{assumption}
This is essentially a coverage assumption on the state-action feature space, which is standard in offline bandits and RL \citep{yin2022near}. The next result bounds the estimation error of  $\hat\theta_{\texttt{SGD-RR}}$ in $\ell_2$-norm.
\begin{theorem}[Estimation error of $\hat\theta_{\texttt{SGD-RR}}$]
\label{thm:sgd_rr}
    Fix $\alpha \in (0,1/e)$ and $\epsilon \ge 0$. Then, under Assumptions~\ref{ass:bound} and~\ref{ass:cov} and setting $\eta_t = \frac{1}{\gamma \kappa}$, we have, with probability at least $1-\alpha$, 
    \begin{align*}
\norm{\hat\theta_{\texttt{SGD-RR}} \!-\! \theta^*}_2 \!\le\! C \!\cdot\! \frac{L}{\gamma \kappa} \!\cdot\!\frac{e^{\epsilon}\!+\!1}{e^{\epsilon}\!-\!1}\!\sqrt{ \frac{\log\left(\log(n)/\alpha\right)}{ n}},
    \end{align*}
where $\gamma = \frac{1}{2 + e^{-2LB} + e^{2LB}}$, $C$ is an absolute constant.
\end{theorem}


 The key idea behind this result is to show the gradient $\hat g_t$ in the SGD update \eqref{eq:estimate_SGD} is an unbiased estimate of the gradient (except some scaling) in the clear-text $g_t = -\nabla_{\hat\theta_t} \log  p_{t,y_t}$, where $p_{t,y}, y \in \lbrace 0,1\rbrace$ denotes the probability of observing $y$ at round $t$, see \eqref{eq:gen-np}.
Specifically, we have
\begin{align*}
        \hat{g}_t = \frac{\sum_{y\in \lbrace 0,1\rbrace} \nabla_{\hat\theta_t} \log  p_{t,y}}{e^{\epsilon} + 1}- \nabla_{\hat\theta_t} \log  p_{t,\widetilde y_t} ~,
    \end{align*}
which, in turn, gives $\mathbb{E}\left [\hat g_t |x_t,y_t,\hat\theta_t\right] \!=\! \left(2\sigma(\epsilon)-1\right)g_t$, where the expectation is over the $\epsilon$-randomization of clear-text label $y_t$ given by \eqref{eq:RR}. This, along with the coverage assumption and the fact that $\sigma'(x_t^\top \theta) \ge \gamma$ for all $\theta \in \Theta_B$ help us achieve the desired error bound. 



\subsection{Proof for SGD}

% We divide the proof of Theorem~\ref{thm:sgd_rr} into the following steps. For ease of presentation, the complete algorithm for computing $\hat\theta_{\texttt{SGD-RR}}$ is given in Algorithm~\ref{alg:LabelDP-main}.

% \textbf{Step 1:} For each $t \ge 1$, we aim to show that there exists some constants $\lambda$, $G$ and random variable $\hat{z}_t$ such that  

Recall that that the gradient at round $t$ is given by
\begin{align*}
        \hat{g}_t = \epsilon\sum_{y\in \lbrace 0,1\rbrace} \nabla_{\hat\theta_t} \log  p_{t,y}- \nabla_{\hat\theta_t} \log  p_{t,\widetilde y_t} ~,
\end{align*}
where $p_{t,y}, y \in \lbrace 0,1\rbrace$ denotes the probability of observing $y$ at round $t$, see \eqref{eq:gen-np}.

Now, we define $\hat{z}_t := \mathbb{E}[\hat{g}_t | \cF_{t-1}] - \hat{g}_t$, where $\cF_{t-1}=\sigma\big(\lbrace x_s,y_s,\widetilde y_s\rbrace_{s=1}^{t-1}\big)$ is the $\sigma$-algebra generated by all the random variables up to and including round $t-1$. This conditioning is necessary since $\widehat\theta_t$ depends on randomness till round $t-1$.
Then, we have 
\begin{align}
    \norm{\widehat\theta_{t+1} - \theta^*}^2 &= \norm{\Pi_{\Theta_B}(\widehat\theta_t - \eta_t \hat{g}_t) - \theta^*}^2\nonumber\\
    &\le \norm{\widehat\theta_t - \eta_t \hat{g}_t - \theta^*}^2\nonumber\\
    &= \norm{\widehat\theta_t - \theta^*}^2 - 2 \eta_t \inner{\hat{g}_t}{\widehat\theta_t - \theta^*} + \eta_t^2 \norm{\hat{g}_t}^2 \nonumber\\
    &= \norm{\widehat\theta_t - \theta^*}^2 -2 \eta_t \inner{\mathbb{E}[\hat{g}_t | \cF_{t-1}] }{\widehat\theta_t - \theta^*} + 2\eta_t \inner{\tilde g_t}{\hat\theta_t - \theta^*} + \eta_t^2 \norm{\hat{g}_t}^2\label{eq:goal1-temp}
\end{align}
where the last equality holds by definition of $\tilde g_t$, i.e., $\hat{g}_t = \mathbb{E}[\hat{g}_t | \cF_{t-1}] -\hat  z_t$.

To bound the above, we need to study the term $\inner{\mathbb{E}[\hat{g}_t | \cF_{t-1}] }{\hat\theta_t - \theta^*}$. First note that $\hat{g}_t$ is an unbiased and scaled estimate of the non-noisy gradient $g_t = -\nabla_{\hat\theta_t} \log  p_{t,y_t}$ as 
\begin{align*}
     \mathbb{E}[\hat{g}_t | \cF_{t-1},z_t,y_t]
    &=  \epsilon\sum_{y\in \lbrace 0,1\rbrace} \nabla_{\hat\theta_t} \log  p_{t,y} - \left( (1-\epsilon) \nabla_{\hat\theta_t} \log  p_{t,y_t} + \epsilon \nabla_{\hat\theta_t} \log  p_{t,1-y_t}  \right)\\
    &=-(1-2\epsilon)\nabla_{\hat\theta_t} \log  p_{t,y_t} = (1-2\epsilon)g_t~.
\end{align*}
Then, by tower property of conditional expectation, we have
\begin{align*}
    \mathbb{E}[\hat{g}_t | \cF_{t-1}] = \mathbb{E}[\mathbb{E}[\hat{g}_t | \cF_{t-1},z_t,y_t] | \cF_{t-1}] = (1-2\epsilon)\mathbb{E}[g_t| \cF_{t-1}]= \beta (1-2\epsilon)\mathbb{E}[(\sigma(\beta h_{\hat\theta_t}(z_t))-y_t)\nabla h_{\hat\theta_t}(z_t)| \cF_{t-1}]~,
\end{align*}
where the final equality holds by definition of $g_t$. One more application of tower property gives us
\begin{align*}
    \mathbb{E}[(\sigma(\beta h_{\hat\theta_t}(z_t))-y_t)\nabla h_{\hat\theta_t}(z_t)| \cF_{t-1}] &= \mathbb{E}[\mathbb{E}[(\sigma(\beta h_{\hat\theta_t}(z_t))-y_t)\nabla h_{\hat\theta_t}(z_t)|\cF_{t-1},z_t]| \cF_{t-1}]\\
    &= \mathbb{E}[(\sigma(\beta h_{\hat\theta_t}(z_t))-\sigma(\beta h_{\theta^*}(z_t))\nabla h_{\hat\theta_t}(z_t)|\cF_{t-1}]~.
\end{align*}
Since $\hat\theta_t$ is deterministic given $\cF_{t-1}$, we can bound
$\inner{\mathbb{E}[\hat{g}_t | \cF_{t-1}] }{\hat\theta_t - \theta^*}$ using the above two equation as
\begin{align}
    &\inner{\mathbb{E}[\hat{g}_t | \cF_{t-1}] }{\hat\theta_t - \theta^*}\nonumber\\ &= \beta (1-2\epsilon)\mathbb{E}[\inner{(\sigma(\beta h_{\hat\theta_t}(z_t)) - \sigma(\beta h_{\theta^*}(z_t) )\nabla h_{\hat\theta_t}(z_t)}{\hat\theta_t - \theta^*} |\cF_{t-1}]\nonumber\\
    &\gep{a} \gamma\beta^2(1-2\epsilon) \mathbb{E}[ \inner{(h_{\hat\theta_t}(z_t) -  h_{\theta^*}(z_t) )\nabla h_{\hat\theta_t}(z_t)}{\hat\theta_t - \theta^*} |\cF_{t-1}]\nonumber\\
    & \gep{b} \gamma\beta^2 (1-2\epsilon) \Big( (\hat\theta_{t} - \theta^*)^{\top}\mathbb{E}[\nabla h_{\hat\theta_t}(z_t) \nabla h_{\hat\theta_t}(z_t)^{\top} |\cF_{t-1}](\hat\theta_{t} - \theta^*)-2\alpha_2 \inner{\mathbb{E}[\nabla h_{\hat\theta_t}(z_t)|\cF_{t-1}]}{\hat\theta_t -\theta^*}\norm{\hat\theta_t -\theta^*}^2\Big)\nonumber\\
    &\gep{c}\gamma\beta^2 (1-2\epsilon) (\kappa -4\alpha_1\alpha_2B)\norm{\hat\theta_t -\theta^*}^2~.\label{eq:gt-bound}
\end{align}
Here (a) holds by mean-value theorem and by noting that $\sigma'(\beta h_{\theta}(z_t)) \ge \gamma$ for all $\theta \in \Theta_B$ under Assumption~\ref{ass:bound}, where $\gamma = \frac{1}{2 + \exp(-2\beta\alpha_0) + \exp(2\beta\alpha_0)}$; (c) holds by Assumption~\ref{ass:cov} and by noting that $\nabla h_{\hat\theta_t}(z_t)$ is independent of $\cF_{t-1}$; (b) holds by first order Taylor expansion for some $\theta \in \Theta_B$
\begin{align*}
  & h_{\theta^*}(z_t) = h_{\hat\theta_t}(z_t) + \inner{\nabla h_{\hat\theta_t}(z_t)}{\theta^*-\hat\theta_t} + (\theta^*-\hat\theta_t)^\top \nabla^2 h_{\theta}(z_t) (\theta^*-\hat\theta_t)\\
  & \implies h_{\hat\theta_t}(z_t)- h_{\theta^*}(z_t) = \inner{\nabla h_{\hat\theta_t}(z_t)}{\hat\theta_t-\theta^*} - (\theta^*-\hat\theta_t)^\top \nabla^2 h_{\theta}(z_t) (\theta^*-\hat\theta_t) \ge \inner{\nabla h_{\hat\theta_t}(z_t)}{\hat\theta_t-\theta^*}-2\alpha_2\norm{\hat\theta_t-\theta^*}^2
\end{align*}
Now, plugging~\eqref{eq:gt-bound} into~\eqref{eq:goal1-temp}, yields 
\begin{align*}
     \norm{\hat\theta_{t+1} - \theta^*}^2 &\le \norm{\hat\theta_t - \theta^*}^2(1 -2\eta_t \gamma\beta^2 (1-2\epsilon) (\kappa -4\alpha_1\alpha_2B)) + 2\eta_t \inner{\tilde g_t}{\hat\theta_t - \theta^*} + \eta_t^2 \norm{\hat{g}_t}^2\\
     &\lep{a} \norm{\hat\theta_t - \theta^*}^2(1 -2\eta_t \gamma\beta^2 (1-2\epsilon) (\kappa -4\alpha_1\alpha_2B)) + 2\eta_t \inner{\tilde g_t}{\hat\theta_t - \theta^*} + \eta_t^2 G^2\\
     &\ep{b}  (1-2/t)\norm{\hat\theta_{t} - \theta^*}^2 + \frac{2}{\lambda t} \inner{\tilde g_t}{\hat\theta_t - \theta*} + \left(\frac{G}{\lambda t}\right)^2
\end{align*}
where (a) holds by bounding $\norm{\hat{g}_t} \le G := 4L $ under Assumption~\ref{ass:bound}; (b) holds by letting $\lambda := \gamma\beta^2 (1-2\epsilon) (\kappa -4\alpha_1\alpha_2B)$ and $\eta_t:= \frac{1}{\lambda t}$; Hence, we have established
\begin{align}
\label{e(1-\epsilon):goal1}
\norm{\widehat\theta_{t+1} - \theta^*}^2 \le (1-2/t)\norm{\widehat\theta_{t} - \theta^*}^2 + \frac{2}{\lambda t} \inner{\tilde g_t}{\hat\theta_t - \theta^*} + \left(\frac{G}{\lambda t}\right)^2.
\end{align}
This gives us
\begin{align}
\label{eq:goal2}
\norm{\hat\theta_{t+1} - \theta^*}^2 \le \frac{2}{\lambda (t-1) t}\sum_{i=2}^t (i-1)\inner{\tilde g_i}{\hat\theta_i - \theta^*} + \frac{G^2}{\lambda^2 t^2}.
\end{align}


We will apply one particular version of Freedman's inequality to control the concentration of $\sum_{i=2}^t (i-1)\inner{\tilde g_i}{\hat\theta_i - \theta^*}$ in~\eqref{eq:goal2}. 

To start with, we let $X_i = \inner{\tilde g_i}{\hat\theta_i -\theta^*}$. Then, we have the conditional expectation of $X_i$ given $\cF_{i-1}$ is $\mathbb{E}[X_i |\cF_{i-1}] = 0$ and the conditional variance is $\text{Var}[X_i |\cF_{i-1}] \le 4G^2 \norm{\hat\theta_i -\theta^*}^2$, which holds by $\norm{\tilde g_i} \le 2G$.
Now consider the sum $\sum_{i=2}^t (i-1)\inner{\tilde g_i}{\theta_i - \theta^*}$ in~\eqref{eq:goal2}. We need to check two conditions: (i) The sum of conditional variance satisfies
\begin{align*}
    \sum_{i=2}^t \text{Var}[(i-1)X_i |\cF_{i-1}] \le 4G^2 \sum_{i=2}^t (i-1)^2 \norm{\hat\theta_i - \theta^*}^2~;
\end{align*}
(ii) Uniform upper bound on each term satisfies
\begin{align*}
   |(i-1)X_i| \le 2G (t-1)\norm{\hat\theta_i - \theta^*} \lep{a} \frac{2G^2 (t-1)}{\lambda},
\end{align*}
where (a) comes from~\eqref{eq:gt-bound} and substituting the value of $\lambda$. To see this, by Cauchy-Schwartz inequality, we have $ \gamma\beta^2 (1-2\epsilon) (\kappa -4\alpha_1\alpha_2B) \norm{\hat\theta_t - \theta^*}^2 \le G \norm{\hat\theta_t - \theta^*}$, and hence $\norm{\hat\theta_t - \theta^*} \le G/\lambda$ for all $t$. We can then apply~\cite{rakhlin2011making} to obtain that for $n \ge 4$ and $\alpha \in (0,1/e)$, with probability at least $1-\delta$, it holds for all $t \le n$ that
\begin{align}
\label{eq:goal3}
    \sum_{i=2}^t (i-1)X_i \le 8G \max\left\{\sqrt{\sum_{i=2}^t (i-1)^2 \norm{\hat\theta_i - \theta^*}^2}, \frac{G(t-1)}{\lambda}\sqrt{\log(\log n/\alpha)}\right\}\sqrt{\log(\log n/\delta)}.
\end{align}

Once we obtain~\eqref{eq:goal3}, the remaining step is all about induction and algebra, which follows the same procedures as in~\cite{rakhlin2011making}. After all, we will obtain with probability at least $1-\delta$ that for all $t \le n$,
\begin{align*}
    \norm{\hat\theta_{t+1} - \theta^*}^2 &\le \frac{(624\log(\log n/\delta)+1)G^2}{\lambda^2 t}\\
    &=C L^2  \frac{\log(\log n/\delta)+1}{\gamma^2 \beta^4(1-2\epsilon)^2(\kappa-4\alpha_1\alpha_2 B)^2 t},
\end{align*}
for some absolute constant $C$. Setting $t=n$ completes the proof.


==> rebuttal.tex <==
\section*{Rebuttal}

We thank the reviewers for their meaningful comments.

\paragraph{Reviewer uvSx}

**SFT policy which provides good coverage of feature space: Practical consideration**  

It has been observed in practice that the generation quality of language model policy obtained using DPO or RLHF depends on the quality of initial SFT policy. The better the generations of the SFT policy, the better the generations of DPO policy. Several recent work have pointed out this fact [R1]. Theoretically, as we argue in Section 4.2, it boils down to ensuring that the minimum eigenvalue of feature covariance matrix under SFT policy is bounded away from zero.


[R1] KTO: Model Alignment as Prospect Theoretic Optimization. Kawin Ethayarajh, Winnie Xu, Niklas Muennighoff, Dan Jurafsky,  Douwe Kiela. https://arxiv.org/pdf/2402.01306.pdf


**Data Efficiency of rDPO v/s DPO v/s RLHF under a fixed noise level**

We can obtain a bound on sample complexity of rDPO for a given noise level and a permissble sub-optimality gap using Theorem 4.4. For instance, consider the log-linear policy class and assume that sample feature covariance matrix $\hat \Sigma$ is invertible. Then, training rDPO on $n \ge \frac{\kappa d}{\Delta^2 \gamma^2 \beta^2(1-2\epsilon)^2}$ samples, we can ensure a sub-optimality gap $\le \Delta$. In contrast, when samples are clean ($\epsilon=0$), then training vanilla DPO on $n \ge \frac{\kappa d}{\Delta^2 \gamma^2 \beta^2}$ samples, we can ensure a suboptimality gap $\le \Delta$. Thus, under the presence of noise, rDPO needs roughly $\frac{1}{(1-2\epsilon)^2}$ times the samples that DPO needs under clean data.



**Choice between SFT and RLHF under a given noise level**

Thanks for pointing out this interesting question. We know that vanilla DPO (or RLHF) policy performs better than SFT policy in datasets like Anthropic-HH, which is known to be noisy. That being said, it remains open to design a noise robust SFT policy and study its performance compared to RLHF policy.


\textbf{Reviewer FRun}

*Dataset diversity and Evaluation model*

We have scaled up the experiments on Anthropic-HH dataset with Llama-7B as language model and GPT4 as evaluation model. We repeat the same procedure as given in the paper to tune the noise rate $\epsilon$ and observe $\epsilon=0.1$ works best. We observe the following comparative performance of rDPO (our method), vanilla DPO and cDPO.

% Table %
We observe that win-rate of rDPO is 5\% higher than vanilla DPO and 7\% higher than cDPO, which explains our method is more tolerant to noisy preferences compared to DPO and cDPO. 

Note that these results are also inline with that reported in Table 3 of the paper. Both these results together asserts versatility of our approach across different models.

*Other SOTA methods*


\textbf{Reviewer xGpp}

*Problem Setup* The limitations language model policy training using RLHF under preference noise is well-documented [R1, R2]. As we have already mentioned in the paper, [R3] propose an approach to estimate the percentage of preference flips in Anthropic-HH dataset and demonstrate the sensitivity of RLHF policy to noisy preferences. They consider the same random noise model like us (see Eq. 8 in the paper) and propose a conservative RLHF/PPO method (cPPO) to mitigate the effect of the noise. [R4] also considers the same problem setup and propose a conservative DPO (cDPO) method. Hence, we believe that this is an important problem to consider, which arises naturally in practical preference datasets like Anthropic-HH. 

Note that the above-mentioned baselines are heuristics and lack theoretical understanding, while we prove sub-optimality gap bound for our method rDPO. We also show improved empirical performance over the baselines on Anthropic-HH and IMDb data.



[R1] Open Problems and Fundamental Limitations of Reinforcement Learning from Human Feedback. Stephen Casper et al. https://arxiv.org/abs/2307.15217 

[R2] Lambert, N., Krendl Gilbert, T., and Zick, T. The history
and risks of reinforcement learning and human feedback.
arXiv e-prints, pp. arXiv–2310, 2023

[R3] Wang, B., Zheng, R., Chen, L., Liu, Y., Dou, S., Huang, C.,
Shen, W., Jin, S., Zhou, E., Shi, C., et al. Secrets of rlhf
in large language models part ii: Reward modeling. arXiv
preprint arXiv:2401.06080, 2024.

[R4] Mitchell, E. A note on dpo with noisy preferences
and relationship to ipo, 2023. URL https://
ericmitchell.ai/cdpo.pdf.


*Section 3.1 and Fact 3.1*

Thank you for the valuable writing suggestions. We will rewrite Fact 3.1 in a straightforward way as:

``It holds that $\mathbb{E}\left[\mathcal{L}_\epsilon(\theta;s,\widetilde a_w,\widetilde a_l)\right] \neq \mathcal{L}(\theta;s, a_w, a_l) $, which makes the BCE loss unbiased under noise." 


Then, in the text we will mention the following: 

`` It also holds that
\begin{align*}
 \text{logit}(\mathbb{P}_{\theta,\epsilon}[a \succ a' |s]) \neq  \text{logit}( \mathbb{P}_{\theta}[a \succ a' |s]). 
\end{align*}
That is the log-odds of preferring $a$ over $a'$ under noisy preferences is different than the corresponding log-odds of that without noise, which introduces a bias in preferences and hence, undesirable."

Then, we continue from the current version

`` Ideally, we want...."


 


*Variance of our rDPO Loss function*

We thank the reviewer for raising this important point and for suggesting to analyze the variance of our unbiased estimator.

Let's consider the un-normalized rDPO loss (we omit the normalizing factor $(1-2\epsilon)$, which anyway doesn't affect the loss-minimizing policy) 
\begin{equation*}
\hat{\mathcal{L}}_\epsilon(\theta;s,\widetilde a_w,\widetilde a_l) =  (1-\epsilon)\mathcal{L}(\theta;s,\widetilde a_w,\widetilde a_l) - \epsilon \mathcal{L}(\theta;s, \widetilde a_l,\widetilde a_w)~.  
\end{equation*}


% minimizing this loss is equivalent to minimizing rDPO loss (Eq. 12 in the paper).

First, observe that
\begin{align*}
     \text{Var}\left[ \hat{\mathcal{L}}_\epsilon(\theta;s,\widetilde a_w,\widetilde a_l)\right] &= \mathbb{E} \left[ \hat{\mathcal{L}}_\epsilon(\theta;s,\widetilde a_w,\widetilde a_l)^2\right] - \mathbb{E} \left[ \hat{\mathcal{L}}_\epsilon(\theta;s,\widetilde a_w,\widetilde a_l)\right]^2
\end{align*}
From Lemma 3.2, we have 
\begin{align*}
 \mathbb{E} \left[ \hat{\mathcal{L}}_\epsilon(\theta;s,\widetilde a_w,\widetilde a_l)\right] = (1-2\epsilon) \mathcal{L}(\theta;s, a_w,a_l)~.   
\end{align*}
From the definition of the rDPO loss, we also have
\begin{align*}
\mathbb{E} \left[ \hat{\mathcal{L}}_\epsilon(\theta;s,\widetilde a_w,\widetilde a_l)^2\right] &=  (1-\epsilon)^2 \mathbb{E} \left[ \mathcal{L}(\theta;s,\widetilde a_w,\widetilde a_l)^2   \right] + \epsilon^2 \mathbb{E} \left[ \mathcal{L}(\theta;s,\widetilde a_l,\widetilde a_w)^2   \right] -2\epsilon (1-\epsilon)  \mathbb{E} \left[ \mathcal{L}(\theta;s,\widetilde a_w,\widetilde a_l)\mathcal{L}(\theta;s,\widetilde a_l,\widetilde a_w)   \right]
\end{align*}
Further, note that
\begin{align*}
&\mathbb{E} \left[ \mathcal{L}(\theta;s,\widetilde a_w,\widetilde a_l)^2   \right] = (1-\epsilon) \mathcal{L}(\theta;s, a_w,a_l)^2 + \epsilon \mathcal{L}(\theta;s, a_l,a_w)^2 \\
&\mathbb{E} \left[ \mathcal{L}(\theta;s,\widetilde a_l,\widetilde a_w)^2   \right] = (1-\epsilon) \mathcal{L}(\theta;s, a_l,a_w)^2 + \epsilon \mathcal{L}(\theta;s, a_w,a_l)^2\\
&\mathbb{E} \left[ \mathcal{L}(\theta;s,\widetilde a_w,\widetilde a_l)\mathcal{L}(\theta;s,\widetilde a_l,\widetilde a_w)   \right] = \mathcal{L}(\theta;s, a_w, a_l)\mathcal{L}(\theta;s, a_l, a_w)
\end{align*}
Combining all these, we get
\begin{align*}
\mathbb{E} \left[ \hat{\mathcal{L}}_\epsilon(\theta;s,\widetilde a_w,\widetilde a_l)^2\right] = (1-3\epsilon+3\epsilon^2) \mathcal{L}(\theta;s, a_w,a_l)^2 + \epsilon (1-\epsilon) \mathcal{L}(\theta;s, a_l,a_w)^2 -2\epsilon (1-\epsilon)  \mathcal{L}(\theta;s, a_w, a_l)\mathcal{L}(\theta;s, a_l, a_w) 
\end{align*}
Then the variance of the rDPO loss is given by
\begin{align*}
    &\text{Var}\left[ \hat{\mathcal{L}}_\epsilon(\theta;s,\widetilde a_w,\widetilde a_l)\right]\\ 
    &= \left[(1-3\epsilon +3\epsilon^2) -(1-2\epsilon)^2\right] \mathcal{L}(\theta;s, a_w,a_l)^2 + \epsilon (1-\epsilon) \mathcal{L}(\theta;s, a_l,a_w)^2 -2\epsilon (1-\epsilon)  \mathcal{L}(\theta;s, a_w, a_l)\mathcal{L}(\theta;s, a_l, a_w)\\
    & = \epsilon (1-\epsilon)\left[\mathcal{L}(\theta;s, a_w,a_l)^2+\mathcal{L}(\theta;s, a_l,a_w)^2-2\mathcal{L}(\theta;s, a_w,a_l)\mathcal{L}(\theta;s, a_l,a_w)\right]\\
    &= \epsilon (1-\epsilon)\left[\mathcal{L}(\theta;s, a_w,a_l)-\mathcal{L}(\theta;s, a_l,a_w)\right]^2.
\end{align*}


 


For the Neural policy class and assuming boundedness, the variance is of the order $O(\alpha_0^2\epsilon(1-\epsilon)) = O (\frac{\alpha_0^2}{4})$ for some constant $\alpha_0$ (see Assumption 4.1 in the paper). Hence, the variance of the loss is bounded and has nice concentration property by Bernstein's inequality. Indeed, we crucially use this fact to bound the estimation error of policy parameter (Theorem 4.2), which eventually yields a bound on the sub-optimality gap (Theorem 4.4).

We will update Lemma 3.2 with the variance bound and put a short discussion about its significance in the text that follows.

 








*Experiments on Anthropic-HH dataset*





 




